Cluster-Based Time-Variant Channel Characterization and Modeling for 5G-Railways

With the development of high-speed railways, 5G for Railways (5G-R) is gradually replacing Global System for the Mobile Communications for Railway (GSM-R) worldwide to meet increasing demands. The large bandwidth, array antennas, and non-stationarity caused by high mobility has made 5G-R channel characterization more complex. Therefore, it is essential to develop an accurate channel model for 5G-R. However, researches on channel characterization and time-variant models specific to 5G-R frequency bands and scenarios is scarce. There are virtually no cluster-based time-variant channel models that capture statistical properties of 5G-R channel. In this paper, we propose a cluster-based time-variant channel model for 5G-R within an enhanced 3GPP framework, which incorporates time evolution features. Extensive channel measurements are conducted on 5G-R private network test line in China. We then extract and analyze typical channel fading characteristics and multipath cluster characteristics. Furthermore, birth-death process of the clusters is modeled by using a four-state Markov chain. Finally, a generalized clustered delay line (CDL) model is established in accordance with 3GPP standard and validated by comparing the results of measurements and simulations. This work enhances the understanding of 5G-R channels and presents a flexible cluster-based time-variant channel model. The results can be used in the design, deployment, and optimization of 5G-R networks.

==> reference.tex <==
%\documentclass[lettersize,journal]{IEEEtran}
%\usepackage{amsmath,amsfonts}
\bibliographystyle{IEEEtran}
%\begin{document}


\nocite{*}

\bibliography{ref}

%\end{document}
  




